Zero-Shot Question Generation from Knowledge Graphs for Unseen Predicates and Entity Types

We present a neural model for question generation from knowledge base triples in a "Zero-Shot" setup, that is generating questions for triples containing predicates, subject types or object types that were not seen at training time. Our model leverages triples occurrences in the natural language corpus in an encoder-decoder architecture, paired with an original part-of-speech copy action mechanism to generate questions. Benchmark and human evaluation show that our model sets a new state-of-the-art for zero-shot QG.

==> Zeroshot Question Generation/figures/copyactions.tex <==


\begin{table}[t]
\centering
\footnotesize 
\begin{tabular}{@{}ll@{}}
\midrule[1.1pt]
\multicolumn{2}{l}{What caused the \texttt{{[}C1\_NOUN{]}} of the \texttt{{[}C3\_NOUN{]}} \texttt{{[}S{]}} ?} \\ \midrule[1pt]
{\multirow{2}{*}{C1}} & \texttt{{[}S{]} \textbf{death} by {[}O{]}} \\                                           \cmidrule(l){2-2}
                      & \texttt{{[}S{]} \textbf{{[}C1\_NOUN{]}} {[}C1\_ADP{]} {[}O{]}} \\                    \midrule[1pt]
{\multirow{2}{*}{C2}} & {Disease} \\ \cmidrule(l){2-2} 
                      & \texttt{{[}C2\_NOUN{]}}               \\\midrule[1pt]
{\multirow{2}{*}{C3}} & {Musical \textbf{artist}}           \\ \cmidrule(l){2-2}
                      & \texttt{{[}C3\_ADJ{]}} \textbf{{\texttt{[}C3\_NOUN{]}}} \\ \bottomrule
\end{tabular}
\caption{An annotated example of part-of-speech copy actions from several input textual contexts (C1, C2, C3), the words or placeholders in bold are copied in the generated question}
\label{table:copyactions}
\end{table}

==> Zeroshot Question Generation/figures/dataset_overlap_stats.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lc}
\hline
          & overlap \% \\ \hline
Sub Type  & 14\%       \\
Obj Type  & 27\%       \\
Predicate & 30\%       \\ \hline
\end{tabular}
\caption{Percentage of textual contexts that has an overlap with the target question}
\label{table:dataset_overlap}
\end{table}

==> Zeroshot Question Generation/figures/dataset_size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

\setlength\extrarowheight{2pt} % or whatever amount is appropriate

\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}l@{\hskip -0.08pt}llll@{}}
\toprule
                                                     &            & \textbf{Train} & \textbf{Valid} & \textbf{Test} \\ \midrule
\raisebox{-.95\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\textbf{\footnotesize{pred}}}}
& \# pred  & 169.4 & 24.2 & 48.4 \\
\multicolumn{1}{l}{}  & \# samples & 55566.7 & 7938.1 & 15876.2 \\
\multicolumn{1}{l}{}  & \% samples & 70.0 $\pm$ 2.77 & 10.0 $\pm$ 1.236 & 20.0 $\pm$ 2.12 \\
\midrule
%%%%%%%%%%%%%%%%
\raisebox{-.95\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\textbf{\footnotesize{sub-types}}}}
& \# types  & 112.7 & 16.1 & 32.2 \\
\multicolumn{1}{l}{}  & \# samples & 60002.6 & 8571.8 & 17143.6 \\
\multicolumn{1}{l}{}  & \% samples & 70.0 $\pm$ 7.9 & 10.0 $\pm$ 3.6 & 20.0 $\pm$ 6.2 \\ \midrule

%%%%%%%%%%%%%%%
\raisebox{-.95\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\textbf{\footnotesize{obj-types}}}} 
& \# types  & 521.6 & 189.9 & 282.2 \\
\multicolumn{1}{l}{}  & \# samples & 57878.1 & 8268.3 & 16536.6 \\
\multicolumn{1}{l}{}  & \% samples & 70.0 $\pm$ 4.7 & 10.0 $\pm$ 2.5 & 20.0 $\pm$ 3.8 \\
\bottomrule
\end{tabular}
\caption{Dataset statistics across 10 folds for each experiment}
\label{tab:dataset-sizes}
\end{table}

==> Zeroshot Question Generation/figures/dep_examples.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{@{}l@{\hskip -0.1pt}l@{}}
\toprule
\textbf{Freebase Relation}                                                   & \textbf{Predicate Textual Context}                                                  \\ \midrule
person/place\_of\_birth                     & {[}O{]} is birthplace of {[}S{]}                 \\
currency/former\_countries         & {[}S{]} was currency of {[}O{]}                  \\
% fb:dish/cuisine                                  & {[}O{]} dish {[}S{]}                             \\
% fb:airliner\_accident/flight\_origin         & {[}S{]} was flight from {[}O{]}                  \\
% fb:film\_featured\_song/performed\_by            & {[}S{]} is release by {[}O{]}                    \\
airline\_accident/operator               & {[}S{]} was accident for {[}O{]}                 \\
genre/artists                                & {[}S{]} became a genre of {[}O{]}                \\
risk\_factor/diseases                     & {[}S{]} increases likelihood of {[}O{]} \\
book/illustrations\_by              & {[}S{]} illustrated by {[}O{]}                   \\
% fb:theatrical\_lyricist/play\_lyrics\_written & {[}O{]} is play written by {[}S{]}   \\
religious\_text/religion       & {[}S{]} contains principles of {[}O{]} \\ 
spacecraft/manufacturer                & {[}S{]} was spacecraft developed by {[}O{]}     \\
\bottomrule
\end{tabular}
\caption{Table showing an example of textual contexts extracted for freebase predicates}
\label{table:example-dep}
\end{table}

% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabular}{@{}ll@{}}
% \toprule
% Freebase Relation                                                   & Predicate Textual Context                                                  \\ \midrule
% fb:person/place\_of\_birth                     & {[}O{]} is birthplace of {[}S{]}                 \\
% % fb:spacecraft/manufacturer                & {[}S{]} was spacecraft developed by {[}O{]}     \\
% fb:currency/countries\_formerly\_used         & {[}S{]} was currency of {[}O{]}                  \\
% % fb:airline\_accident/flight\_origin         & {[}S{]} was flight from {[}O{]}                  \\
% fb:airline\_accident/operator               & {[}S{]} was accident for {[}O{]}                 \\
% fb:book/interior\_illustrations\_by              & {[}S{]} illustrated by {[}O{]}                   \\
% % fb:risk\_factor/diseases                     & {[}S{]} increases likelihood of {[}O{]} \\
% % fb:theatrical\_lyricist/play\_lyrics\_written & {[}O{]} is play written by {[}S{]}   \\
% \bottomrule
% \end{tabular}
% \caption{Table showing an example of textual contexts extracted for freebase predicates}
% \label{table:example-dep}
% \end{table}

==> Zeroshot Question Generation/figures/eval_unseenpredicates.tex <==
\begin{table*}[]
\footnotesize
\centering
\begin{tabular}{@{}ll|ccccccc@{}}
\toprule
& \textbf{Model} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{ROUGE\textsubscript{L}} & \textbf{METEOR} \\
% &       & valid        & test        & valid        & test        & valid        & test        & valid        & test        & valid        & test       & valid        & test  & valid        & test        \\ \midrule\midrule
\midrule[1.1pt]
%\multirow{4}{*}{pred} 
\multirow{4}{*}{\raisebox{-3\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\textbf{\footnotesize{ Unseen Predicates}}}}}

&  SELECT & 46.81 $\pm$ 2.12 & 38.62 $\pm$ 1.78 & 31.26 $\pm$ 1.9 & 23.66 $\pm$ 2.22 & 52.04 $\pm$ 1.43 & 27.11 $\pm$ 0.74 \\
&  IR  & 48.43 $\pm$ 1.64 & 39.13 $\pm$ 1.34 & 31.4 $\pm$ 1.66 & 23.59 $\pm$ 2.36 & 52.88 $\pm$ 1.24 & 27.34 $\pm$ 0.55 \\
&  IR\textsubscript{COPY} & 48.22 $\pm$ 1.84 & 38.82 $\pm$ 1.5 & 31.01 $\pm$ 1.72 & 23.12 $\pm$ 2.24 & 52.72 $\pm$ 1.26 & 27.24 $\pm$ 0.57 \\
&  R-TRANSE & 49.09 $\pm$ 1.69 & 40.75 $\pm$ 1.42 & 33.4 $\pm$ 1.7 & 25.97 $\pm$ 2.22 & 54.07 $\pm$ 1.31 & 28.13 $\pm$ 0.54 \\
&  R-TRANSE\textsubscript{COPY}& 49.0 $\pm$ 1.76 & 40.63 $\pm$ 1.48 & 33.28 $\pm$ 1.74 & 25.87 $\pm$ 2.23 & 54.09 $\pm$ 1.35 & 28.12 $\pm$ 0.57 \\
&    Encoder-Decoder       & 58.92 $\pm$ 2.05 & 47.7 $\pm$ 1.62  & 38.18 $\pm$ 1.86 & 28.71 $\pm$ 2.35 & 59.12 $\pm$ 1.16 & 34.28 $\pm$ 0.54 \\
\cmidrule(l){2-8}
&  Our-Model      & 60.8  $\pm$ 1.52 & 49.8 $\pm$ 1.37  & 40.32 $\pm$ 1.92 & 30.76 $\pm$ 2.7  & 60.07 $\pm$ 0.9  & 35.34 $\pm$ 0.43 \\
& Our-Model\textsubscript{copy}    & \textbf{62.44} $\pm$ 1.85 & \textbf{50.62} $\pm$ 1.46 & \textbf{40.82} $\pm$ 1.77 & \textbf{31.1} $\pm$ 2.46  & \textbf{61.23} $\pm$ 1.2  & \textbf{36.24} $\pm$ 0.65 \\
%\midrule[1.2pt]
%\multirow{4}{*}{subtype} 
%& SELECT & 48.51 $\pm$ 0.8 & 40.46 $\pm$ 0.84 & 33.34 $\pm$ 1.09 & 26.11 $\pm$ 1.47 & 53.72 $\pm$ 0.89 & 28.01 $\pm$ 0.46 \\
%&  IR   & 49.76 $\pm$ 2.05 & 41.37 $\pm$ 1.93 & 34.37 $\pm$ 2.02 & 27.5 $\pm$ 2.28 & 55.37 $\pm$ 1.64 & 28.75 $\pm$ 0.82 \\      
%&  IR\textsubscript{COPY}  & 50.5 $\pm$ 1.32 & 42.21 $\pm$ 1.23 & 35.15 $\pm$ 1.47 & 28.17 $\pm$ 2.01 & 55.74 $\pm$ 1.27 & 29.09 $\pm$ 0.78 \\
%% & IR\textsubscript{Text}_data_types_posdep_placeholder_250_Epochs & 48.94 $\pm$ 1.93 & 40.82 $\pm$ 1.89 & 33.92 $\pm$ 1.98 & 27.09 $\pm$ 2.23 & 54.9 $\pm$ 1.54 & 28.05 $\pm$ 0.99 \\
%&  R-TRANSE  & 53.86 $\pm$ 0.91 & 45.72 $\pm$ 1.04 & 38.93 $\pm$ 1.36 & 32.41 $\pm$ 1.74 & 59.27 $\pm$ 0.92 & 30.9 $\pm$ 0.53 \\
%&  R-TRANSE\textsubscript{COPY}  & 53.77 $\pm$ 0.9 & 45.63 $\pm$ 1.12 & 38.82 $\pm$ 1.44 & 32.26 $\pm$ 1.81 & 59.21 $\pm$ 0.95 & 30.82 $\pm$ 0.55 \\
%%%%%%%%%%% 
%&  Encoder-Decoder         & 69.91 $\pm$ 0.89 & 59.31 $\pm$ 1.21 & 50.56 $\pm$ 1.58 & 42.14 $\pm$ 2.05 & 68.95 $\pm$ 0.86 & 40.65 $\pm$ 0.63 \\ 
%\cmidrule(l){2-8}
%&  + Textual Evidence      & 70.17 $\pm$ 1.02 & 59.49 $\pm$ 1.24 & 50.64 $\pm$ 1.51 & 42.13 $\pm$ 1.88 & 69.35 $\pm$ 0.9 & 40.93 $\pm$ 0.58 \\
%&  + Copy Actions          & \textbf{70.62} $\pm$ 1.13 & \textbf{59.76} $\pm$ 1.29 & \textbf{50.8} $\pm$ 1.58 & \textbf{42.2} $\pm$ 2.0 & \textbf{69.37} $\pm$ 1.0 & \textbf{41.05} $\pm$ 0.67 \\
%% & + POS Copy Actions  & 70.18 $\pm$ 1.03 & 59.44 $\pm$ 1.3 & 50.56 $\pm$ 1.62 & 42.01 $\pm$ 2.04 & 69.09 $\pm$ 1.02 & 40.42 $\pm$ 0.64 \\
%\midrule[1.2pt]
%\multirow{4}{*}{objtype} 
%& SELECT & 44.66 $\pm$ 1.36 & 36.84 $\pm$ 1.25 & 29.77 $\pm$ 1.31 & 22.39 $\pm$ 1.37 & 50.06 $\pm$ 1.02 & 26.0 $\pm$ 0.33 \\
%&  IR   & 48.14 $\pm$ 2.26 & 39.86 $\pm$ 2.32 & 32.76 $\pm$ 2.41 & 25.66 $\pm$ 2.6 & 53.61 $\pm$ 2.22 & 27.87 $\pm$ 1.24 \\
%&  IR\textsubscript{COPY}  & 48.84 $\pm$ 2.28 & 40.45 $\pm$ 2.21 & 33.35 $\pm$ 2.2 & 26.28 $\pm$ 2.31 & 54.22 $\pm$ 2.12 & 28.04 $\pm$ 1.23 \\                                                           
%% & IR\textsubscript{TransE}_data_types_posdep_placeholder_250_Epochs & 50.81 $\pm$ 0.98 & 42.72 $\pm$ 1.17 & 36.05 $\pm$ 1.35 & 29.62 $\pm$ 1.56 & 56.82 $\pm$ 1.18 & 28.57 $\pm$ 0.92 \\                              
%&  R-TRANSE  & 51.99 $\pm$ 0.9 & 43.89 $\pm$ 0.96 & 37.13 $\pm$ 1.1 & 30.59 $\pm$ 1.3 & 57.37 $\pm$ 1.17 & 29.86 $\pm$ 0.67 \\
%&  R-TRANSE\textsubscript{COPY}  & 51.95 $\pm$ 0.63 & 43.73 $\pm$ 0.85 & 36.9 $\pm$ 1.1 & 30.32 $\pm$ 1.38 & 57.45 $\pm$ 0.94 & 29.87 $\pm$ 0.53 \\                                                                                                                  
%% & IR\textsubscript{Text}_data_types_posdep_placeholder_250_Epochs & 48.14 $\pm$ 2.31 & 39.88 $\pm$ 1.93 & 32.92 $\pm$ 1.83 & 25.98 $\pm$ 1.94 & 53.74 $\pm$ 2.04 & 27.57 $\pm$ 1.34 \\                                                                                    
%&  Encoder-Decoder          & 66.24 $\pm$ 1.99 & 55.51 $\pm$ 2.35 & 46.5 $\pm$ 2.54 & 37.79 $\pm$ 2.65 & 65.69 $\pm$ 2.25 & 38.31 $\pm$ 1.75 \\                      
%\cmidrule(l){2-8}
%& + Textual Evidence        & 66.54 $\pm$ 1.33 & 55.75 $\pm$ 1.69 & 46.65 $\pm$ 1.88 & 37.78 $\pm$ 2.02 & 65.51 $\pm$ 1.56 & 38.31 $\pm$ 1.28 \\
%& + Copy Actions            & \textbf{67.68} $\pm$ 1.04 & \textbf{56.34} $\pm$ 1.54 & \textbf{47.02} $\pm$ 1.75 & \textbf{38.02} $\pm$ 1.9 & \textbf{66.24} $\pm$ 1.38 & \textbf{38.87} $\pm$ 0.98 \\
%% & + POS Copy Actions  & 67.11 $\pm$ 1.05 & 55.85 $\pm$ 1.55 & 46.5 $\pm$ 1.81 & 37.46 $\pm$ 1.99 & 65.87 $\pm$ 1.44 & 38.1 $\pm$ 1.05 \\
\bottomrule
\end{tabular}
\caption{\small{Evaluation results of our model and all other baselines for the unseen predicate evaluation setup}}
\label{table:eval-pred}
\end{table*}
%
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}ll|cc@{}}
\toprule
& \textbf{Model} & \textbf{BLEU-4} & \textbf{ROUGE\textsubscript{L}} \\
\midrule[1.1pt]
%\multirow{4}{*}{subtype} 
\multirow{4}{*}{\raisebox{-0.6\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\textbf{\footnotesize{Sub-Types}}}}}
% & SELECT & 26.11 $\pm$ 1.47 & 53.72 $\pm$ 0.89 \\
%&  IR   & 27.5 $\pm$ 2.28 & 55.37 $\pm$ 1.64 \\
%&  IR\textsubscript{COPY}  & 28.17 $\pm$ 2.01 & 55.74 $\pm$ 1.27 \\
%% & IR\textsubscript{Text}_data_types_posdep_placeholder_250_Epochs & 48.94 $\pm$ 1.93 & 40.82 $\pm$ 1.89 & 33.92 $\pm$ 1.98 & 27.09 $\pm$ 2.23 & 54.9 $\pm$ 1.54 & 28.05 $\pm$ 0.99 \\
&  R-TRANSE  & 32.41 $\pm$ 1.74 & 59.27 $\pm$ 0.92 \\
%&  R-TRANSE\textsubscript{COPY}  & 32.26 $\pm$ 1.81 & 59.21 $\pm$ 0.95 \\
%%%%%%%%%% 
&  Encoder-Decoder         & 42.14 $\pm$ 2.05 & 68.95 $\pm$ 0.86 \\
\cmidrule(l){2-4}
& Our-Model                       & 42.13 $\pm$ 1.88 & 69.35 $\pm$ 0.9 \\
& Our-Model\textsubscript{copy}   & \textbf{42.2} $\pm$ 2.0 & \textbf{69.37} $\pm$ 1.0 \\
% & + POS Copy Actions  & 70.18 $\pm$ 1.03 & 59.44 $\pm$ 1.3 & 50.56 $\pm$ 1.62 & 42.01 $\pm$ 2.04 & 69.09 $\pm$ 1.02 & 40.42 $\pm$ 0.64 \\
\midrule[1.2pt]
%\multirow{4}{*}{objtype} 
\multirow{4}{*}{\raisebox{-0.6\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\textbf{\footnotesize{Obj-Types}}}}}
% & SELECT & 22.39 $\pm$ 1.37 & 50.06 $\pm$ 1.02 \\
%&  IR   & 25.66 $\pm$ 2.6 & 53.61 $\pm$ 2.22 \\
%&  IR\textsubscript{COPY}  & 26.28 $\pm$ 2.31 & 54.22 $\pm$ 2.12 \\                                                          
%% & IR\textsubscript{TransE}_data_types_posdep_placeholder_250_Epochs & 50.81 $\pm$ 0.98 & 42.72 $\pm$ 1.17 & 36.05 $\pm$ 1.35 & 29.62 $\pm$ 1.56 & 56.82 $\pm$ 1.18 & 28.57 $\pm$ 0.92 \\                              
&  R-TRANSE  & 30.59 $\pm$ 1.3 & 57.37 $\pm$ 1.17 \\
%&  R-TRANSE\textsubscript{COPY}  & 30.32 $\pm$ 1.38 & 57.45 $\pm$ 0.94 \\                                                                                                             
%% & IR\textsubscript{Text}_data_types_posdep_placeholder_250_Epochs & 48.14 $\pm$ 2.31 & 39.88 $\pm$ 1.93 & 32.92 $\pm$ 1.83 & 25.98 $\pm$ 1.94 & 53.74 $\pm$ 2.04 & 27.57 $\pm$ 1.34 \\                                                                                    
&  Encoder-Decoder          & 37.79 $\pm$ 2.65 & 65.69 $\pm$ 2.25 \\                      
\cmidrule(l){2-4}
& Our-Model        & 37.78 $\pm$ 2.02 & 65.51 $\pm$ 1.56 \\
& Our-Model\textsubscript{copy}            & \textbf{38.02} $\pm$ 1.9 & \textbf{66.24} $\pm$ 1.38 \\
% & + POS Copy Actions  & 67.11 $\pm$ 1.05 & 55.85 $\pm$ 1.55 & 46.5 $\pm$ 1.81 & 37.46 $\pm$ 1.99 & 65.87 $\pm$ 1.44 & 38.1 $\pm$ 1.05 \\
\bottomrule
\end{tabular}
\caption{\small{Automatic evaluation of our model against selected baselines for unseen sub-types and obj-types}}
\label{table:eval-type}
\end{table}

==> Zeroshot Question Generation/figures/qualitative_eval.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}l@{\hskip -3pt}cc@{}}
\toprule
\textbf{Model} & \textbf{$\%$ Pred. Identified}    & \textbf{Natural.} \\ \midrule
Encoder-Decoder                 & $6$                &   $3.14$          \\
Our-Model (No Copy)         & $6$                &   $2.72$          \\
Our-Model\textsubscript{copy} (Types context) & $\mathbf{37}$      &    $\mathbf{3.21}$         \\
Our-Model\textsubscript{copy} (All contexts)       & $\mathbf{46}$ & $2.61$           \\ \midrule
% Reference       &  --  & $\mathbf{4.32}$            \\ \bottomrule
\end{tabular}
\caption{results of Human evaluation on \% of predicates identified and naturalness 0-5}
\label{table:human-eval}
\end{table}


==> Zeroshot Question Generation/figures/results_examples.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabularx}{1.05\linewidth}{l|lX} 
\toprule
1&\textbf{Reference} & \textbf{what language is spoken in the tv show three sheets?}                                      \\
&\textbf{Enc-Dec.}   & in what \textbf{language} is three sheets in?                                    \\
&\textbf{Our-Model}        & what the the player is the three sheets?                           \\
&\textbf{Our-Model\textsubscript{Copy}}      & what is the \textbf{language} of three sheets? \\\midrule
2&\textbf{Reference} & \textbf{how is roosevelt in Africa classified?                        } \\
&\textbf{Enc-Dec.}   & what is the name of a roosevelt in Africa?                    \\
&\textbf{Our-Model}        & what is the name of the movie roosevelt in Africa?               \\
&\textbf{Our-Model\textsubscript{Copy}}     & what is a \textbf{genre} of roosevelt in Africa?                          \\ \midrule
3&\textbf{Reference} & \textbf{where can 5260 philvéron be found}?                              \\
&\textbf{Enc-Dec.}   & what is a release some that 5260 philvéron wrote?                \\
&\textbf{Our-Model}        & what is the name of an artist 5260 philvéron?                    \\
&\textbf{Our-Model\textsubscript{Copy}}     & which \textbf{star system} contains the star system body 5260 philvéron?  \\ \midrule
4&\textbf{Reference} & \textbf{which university did ezra cornell create}?             \\
&\textbf{Enc-Dec.}   & which films are part of ezra cornell?             \\
&\textbf{Our-Model}        & what is a position of ezra cornell?                              \\
&\textbf{Our-Model\textsubscript{Copy}}     & what \textit{founded} the name of a university that ezra cornell \textbf{founded}? \\ 
% 5&\textbf{Reference} & \textbf{who founded snocap , inc .}?                                      \\
% &\textbf{Enc-Dec.}   & which asian snocap is most as?                                \\
% &\textbf{Our model}        & what is the name of a person of snocap?                          \\
% &\textbf{+ Copy}      & who is the \textbf{person behind} snocap?                                 \\ \midrule

% 6&\textbf{Reference} & \textbf{which 1992 album was produced by daniel barenboim?} \\
% &\textbf{Enc-Dec.}   & which german contains daniel barenboim ?  \\
% &\textbf{Our model}  & which \textbf{album} is from the subject daniel barenboim   \\
% &\textbf{+ Copy}      & what was the name of \textit{\textbf{a album}} that is daniel barenboim ? \\
\bottomrule
\end{tabularx}
\caption{Examples of generated questions from different systems in comparison}
\label{table:results-example}
\end{table}

==> Zeroshot Question Generation/figures/training_example.tex <==

\begin{table*}[]
\centering
\small
\setlength\extrarowheight{2pt}
\begin{tabularx}{0.9\linewidth}[t]{lp{0.72\linewidth}}
\noalign{\hrule height 1pt}
% \toprule\toprule
Input Triple &  fb:03cz5\_p fb:executive\_produced\_by fb:0h5t1m8  \\ 
\noalign{\hrule height 0.7pt}
Question &   who produced the film woodstock villa ?\\ 
\noalign{\hrule height 0.7pt}
Textual Evidence &  [[OBJ]] produced [[SUB]] \\ 
\noalign{\hrule height 0.7pt}
Textual Evidence POS &  [[OBJ]] VERB [[SUB]] \\ 
\noalign{\hrule height 0.7pt}
Subject Textual Evidence & Film  \\ 
\noalign{\hrule height 0.7pt}
Object Textual Evidence & Person  \\ 
\noalign{\hrule height 0.7pt}
Question With Special Tokens &  who [[DEP VERB]] the [[SUB TYPE]] [[SUB]] ? \\  
\noalign{\hrule height 1pt}
\end{tabularx}
\caption{An Example showing one training example }
\label{table:main-example}
\end{table*}

==> figures/dataset_overlap_stats.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lc}
\hline
          & overlap \% \\ \hline
Sub Type  & 14\%       \\
Obj Type  & 27\%       \\
Predicate & 30\%       \\ \hline
\end{tabular}
\caption{Percentage of textual contexts that has an overlap with the target question}
\label{table:dataset_overlap}
\end{table}

==> figures/training_example.tex <==

\begin{table*}[]
\centering
\small
\setlength\extrarowheight{2pt}
\begin{tabularx}{0.9\linewidth}[t]{lp{0.72\linewidth}}
\noalign{\hrule height 1pt}
% \toprule\toprule
Input Triple &  fb:03cz5\_p fb:executive\_produced\_by fb:0h5t1m8  \\ 
\noalign{\hrule height 0.7pt}
Question &   who produced the film woodstock villa ?\\ 
\noalign{\hrule height 0.7pt}
Textual Evidence &  [[OBJ]] produced [[SUB]] \\ 
\noalign{\hrule height 0.7pt}
Textual Evidence POS &  [[OBJ]] VERB [[SUB]] \\ 
\noalign{\hrule height 0.7pt}
Subject Textual Evidence & Film  \\ 
\noalign{\hrule height 0.7pt}
Object Textual Evidence & Person  \\ 
\noalign{\hrule height 0.7pt}
Question With Special Tokens &  who [[DEP VERB]] the [[SUB TYPE]] [[SUB]] ? \\  
\noalign{\hrule height 1pt}
\end{tabularx}
\caption{An Example showing one training example }
\label{table:main-example}
\end{table*}
